On Modified Newton Methods for Unconstrained Optimization Based on Lanczos Tridiagonalization

For a strongly convex unconstrained minimization problem, Newton's method with a line search offers rapid convergence to a minimizer by incorporating second-order information. However, for a general unconstrained problem the Hessian need not be positive definite, which can lead to the inability to find a search direction or to search directions that fail to produce descent. Modified Newton methods are designed to handle this situation. This paper considers modifications to a Newton-conjugate-gradient approach based on Lanczos tridiagonalization. Existing methods are extended using dynamic modification schemes that provide a descent direction while keeping the modification bounded. A Lanczos-based scheme and a conjugate-gradient (CG)-based scheme are formulated and analyzed. These methods are mathematically equivalent in exact arithmetic, but their practical behavior differs in finite precision. Finally, it is shown how the convergence and computational cost are affected by varying the amount of additional curvature introduced and by allowing the early termination of the inner iterations.

==> algmacros.tex <==

%\def\tab{\par\indent}
%\def\tabb{\tab\hskip1.5em}
%\def\tabbb{\tab\hskip3.5em}
%\def\tabbbb{\tab\hskip5.5em}
%\def\tabbbbb{\tab\hskip7.5em}

\makeatletter

\newcommand{\ent}[1]{$\pthinsp #1\pthinsp$}
\newcommand{\Percent}{\texttt{\bfseries\%\mgap}}
\newcommand{\algname}[1]{\hbox{\small{\bf\texttt{#1}}}}
%\renewcommand{\algname}[1]{\ensuremath{\textbf{#1}}}
\algrenewcommand{\algorithmiccomment}[1]{\hfill[#1]}
\algnewcommand{\LineComment}[1]{\State[#1]}
%\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\IIf}[1]{\algorithmicif\ #1\  \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}
\algnewcommand{\IFor}[1]{\algorithmicfor\ #1\ \algorithmicdo}
\algnewcommand{\EndIFor}{\unskip\ \algorithmicendfor}
\newcommand{\algorithmicendfor}{\algorithmicend\ \algorithmicfor}
%\algnewcommand{\IElse}[1]{\unskip\ \algorithmicelse\ #1\ \algorithmicend\ \algorithmicif}
\algnewcommand{\IElse}[1]{\unskip\ \algorithmicelse\ #1}
\algnewcommand{\IElseIf}[1]{\algorithmicelse\ \algorithmicif\ #1\  \algorithmicthen}

\newcommand{\Restrictions}[1]{\small{\textbf{Restrictions:}} #1}
\newcommand{\Constants}[1]{\small{\textbf{Constants:}} #1}
\newcommand{\Input}[1]{\textbf{Input:} #1}

\newcommand{\Alg}[1]{\textsf{\bfseries#1}}
%\newcommand{\Sstrut}{\vrule height12pt depth5.5pt width0pt}
\newcommand{\algcomment}[1]{\emph{\Percent#1;}\Cstrut}
\newcommand{\commenta}[1]{\emph{\Percent#1}\Cstrut}  % first line of two-liner
\newcommand{\commentb}[1]{\emph{\Percent#1;}}        % second line
%\newcommand{\Step}[1]{\Sstrut\textit{\bfseries Step~#1:}}
\newcommand{\Step}[1]{\textit{\bfseries Step~#1:}} % mhw

\newcommand{\algstrut}{\rule[-.6ex]{0pt}{3ex}}% Total height 3.6
\renewcommand{\algstrut}{\vrule height12pt depth5.5pt width0pt}
\newcommand{\Astrutu}{\rule{0pt}{2.75ex}}
\newcommand{\astrutu}{\rule{0pt}{2ex}}
\newcommand{\struta}{\rule[-1.25ex]{0pt}{2ex}}%
\newcommand{\strutb}{\rule[-.9ex]{0pt}{2ex}}%
\newcommand{\mystrut}{\vrule height9.5pt depth1.5pt width0pt}

\newcommand{\agap}{\hspace{1.5ex}}
\newcommand{\cgap}{$\;$}   % one thick space
% \newcommand{\AlgSec}[1]{{\bf[#1.]}\vrule height10pt depth1.5pt width0pt}
\newcommand{\AlgSec}[1]{#1\vrule height10pt depth1.5pt width0pt}
%\newcommand{\Comment}[1]{#1\vrule height10pt depth1.5pt width0pt} % mhw

\newcommand{\Delete}{\mathtt{Delete}}
\newcommand{\Swap}{\mathtt{Swap}}
\newcommand{\Add}{\mathtt{Add}}
\newcommand{\return}{\mathtt{return}}

%% %\newcommand{\tab{\par\noindent\struta}
%% %\newcommand{\tab}{\par\noindent\mystrut}   % MHW! we need to talk about
%%                                            % which of these macros to use
%% \newcommand{\tab}{\par\noindent}% mhw
%% \newcommand{\tabalg}{\vskip -2pt\par\noindent}  % mhw
%% \newcommand{\tabprestep}{\vskip 1.5pt\par\noindent}% mhw
%% \newcommand{\tabextrastep}{\vskip 1.7pt\par\noindent}% mhw
%% \newcommand{\tabbprestep}{\vskip 1.5pt\par\noindent\hskip 1.5em}% mhw
%% \newcommand{\tabbalg}{\vskip -1.2pt\tab\hskip 1.5em} % mhw
%% \newcommand{\tabbbalg}{\vskip -1.2pt\tab\hskip 3.5em} % mhw
%% \newcommand{\tablil}{\tab\hskip1em} % mhw
%% \newcommand{\tabbextrastep}{\vskip 1.7pt\tabb}% mhw

%% \newcommand{\tabb}{\tab\hskip1.5em}
%% %\newcommand{\tabb}{\tab\hskip2em} % mhw
%% %\newcommand{\tabbb}{\tab\hskip4em}  % mhw
%% \newcommand{\tabbb}{\tab\hskip3.5em}
%% \newcommand{\tabbbb}{\tab\hskip5.5em}
%% \newcommand{\tabbbbb}{\tab\hskip7.5em}
%% \newcommand{\tabbbbbb}{\tab\hskip9.5em}

%% \newcommand{\alg}[1]{\par\noindent\mystrut\ignorespaces\hbox to\textwidth{#1\hfill}}
%% \newcommand{\algt}[1]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip1.5em#1\hfill}}
%% \newcommand{\algtt}[1]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip3.5em#1\hfill}}
%% \newcommand{\algttt}[1]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip5.5em#1\hfill}}
%% \newcommand{\algtttt}[1]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip7.5em#1\hfill}}
%% \newcommand{\algttttt}[1]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip9.5em#1\hfill}}
%% \newcommand{\clg}[2]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces#1\hfill[#2]}}
%% \newcommand{\clgt}[2]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip1.5em#1\hfill[#2]}}
%% \newcommand{\clgtt}[2]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip3.5em#1\hfill[#2]}}
%% \newcommand{\clgttt}[2]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip5.5em#1\hfill[#2]}}
%% \newcommand{\clgtttt}[2]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip7.5em#1\hfill[#2]}}
%% \newcommand{\clgttttt}[2]{\par\noindent\mystrut\hbox to\textwidth{\ignorespaces\hskip9.5em#1\hfill[#2]}}

\newcommand{\tac}{\par\noindent\mystrut\hskip1em}
%\newcommand{\tabc}{\tab\hskip2.5em}
\newcommand{\tabc}{\tab\hskip2em}  % mhw
\newcommand{\tabcc}{\tab\hskip4.5em}
\newcommand{\tabccc}{\tab\hskip6.5em}
\newcommand{\tabcccc}{\tab\hskip8.5em}
\newcommand{\tabccccc}{\tab\hskip10.5em}

\newcommand{\REPEAT}{\hbox{\bf repeat}\Astrut}
\newcommand{\WHILE}{\hbox{\bf while}\hskip2pt}
\newcommand{\FOR}{\hbox{\bf for}\hskip2pt}
\newcommand{\IF}{\hbox{\bf if}\hskip2pt}

\newcommand{\logical}[1]{\{\ensuremath{#1}\}}
\newcommand{\proc}[1]{\setbox4=\hbox{\noindent\strut#1}\boxit{\box4}}
\newcommand{\procc}[1]{\setbox4=\vbox{\hsize 20pc \noindent\strut#1}\boxit{\box4}}
\newcommand{\DO}{\hskip2pt\hbox{\bf do}\hskip2pt\Astrut}
\newcommand{\UNTIL}{\hbox{\bf until}\hskip2pt}
\newcommand{\BEGIN}{\hbox{\bf begin}}
\newcommand{\END}{\hbox{\bf end}}
\newcommand{\ENDIF}{\hbox{\bf end if}}
\newcommand{\ENDWHILE}{\hbox{\bf end while}}
\newcommand{\ENDREPEAT}{\hbox{\bf end repeat}}
\newcommand{\ENDDO}{\hbox{\bf end do}}
\newcommand{\ENDFOR}{\hbox{\bf end for}} % mhw
\newcommand{\THEN}{\hskip2pt\hbox{\bf then}\hskip2pt}
\newcommand{\ELSE}{\hskip2pt\hbox{\bf else}\hskip2pt}
\newcommand{\ELSEIF}{\hbox{\bf else if}}

\newcommand{\STOP}{\mathsf{stop}}
\newcommand{\Stop}{\mathsf{stop}}
\newcommand{\Fail}{\mathsf{fail}}
\newcommand{\TRUE}{\mathsf{true}}
\newcommand{\FALSE}{\mathsf{false}}
\newcommand{\true}{\mathbf{true}}
\newcommand{\True}{\mathbf{true}}
\newcommand{\false}{\mathbf{false}}
\newcommand{\False}{\mathbf{false}}
\newcommand{\NOT}{\mathop{\mathbf{not}\,}}
\newcommand{\AND}{\mathop{\;\mathbf{and}\;}}
\newcommand{\OR}{\mathop{\;\mathbf{or}\;}}
\newcommand{\BREAK}{\mathbf{break}}
\newcommand{\Break}{\mathbf{break}}

% Pseudo-code only macros

\newcommand{\equals}{\xlongequal{\hspace{2pt}}}
\newcommand{\maxit}{\ensuremath{\mathsf{maxit}}}
\newcommand{\badSteps}{\ensuremath{\mathsf{badSteps}}}
\newcommand{\bracketed}{\ensuremath{\mathsf{bracketed}}}
\newcommand{\converged}{\ensuremath{\mathsf{converged}}}
%\newcommand{\conv}{\ensuremath{\mathsf{converged}}}
\newcommand{\complete}{\ensuremath{\mathsf{complete}}}
\newcommand{\CSpoint}{\ensuremath{\mathsf{subspace\_stationary\_pt}}}
\newcommand{\done}{\ensuremath{\mathsf{done}}}
\newcommand{\exchange}{\ensuremath{\mathsf{exchange}}}
\newcommand{\exit}{\ensuremath{\mathsf{exit}}}
\newcommand{\found}{\ensuremath{\mathsf{found}}}
\newcommand{\feasible}{\ensuremath{\mathsf{feasible}}}
\newcommand{\WolfeStep}{\ensuremath{\mathsf{wolfe\_step}}}
\newcommand{\ArmijoStep}{\ensuremath{\mathsf{armijo\_step}}}
\newcommand{\hitcon}{\ensuremath{\mathsf{hit\_constraint}}}
\newcommand{\Hsingular}{\ensuremath{\mathsf{singular\_H}}}
\newcommand{\imprvd}{\ensuremath{\mathsf{improved}}}
\newcommand{\indef}{\ensuremath{\mathsf{indefinite}}}
\newcommand{\minimizer}{\ensuremath{\mathsf{subspace\_minimizer}}}
\newcommand{\Optimal}{\ensuremath{\mathsf{optimal\_multipliers}}}
\newcommand{\optimal}{\ensuremath{\mathsf{optimal}}}
\newcommand{\posdef}{\ensuremath{\mathsf{positive\_definite}}}
\newcommand{\unbounded}{\ensuremath{\mathsf{unbounded}}}
\newcommand{\semidef}{\ensuremath{\mathsf{positive\_semidefinite}}}
\newcommand{\stationary}{\ensuremath{\mathsf{stationary\_point}}}
\newcommand{\subspace}{\ensuremath{\mathsf{subspace\_convergence}}}
\newcommand{\singular}{\ensuremath{\mathsf{singular}}}
\newcommand{\tol}{\ensuremath{\mathsf{tol}}}
\newcommand{\uncon}{\ensuremath{\mathsf{unconstrained\_step}}}
\newcommand{\vertex}{\ensuremath{\mathsf{vertex}}}
\newcommand{\wschosen}{\ensuremath{\mathsf{working\_set\_chosen}}}
\newcommand{\Wsingular}{\ensuremath{\mathsf{singular\_W}}}
\newcommand{\zeroCurvature}{\ensuremath{\mathsf{zero\_curvature}}}
\newcommand{\SubMin}{\ensuremath{\mathsf{subspace\_minimizer}}}
\newcommand{\addConstraint}{\ensuremath{\mathsf{add\_constraint}}}
\newcommand{\stageone}{\ensuremath{\mathsf{stage\_one}}}
\newcommand{\stagetwo}{\ensuremath{\mathsf{stage\_two}}}
\newcommand{\modulo}{\ensuremath{\mathsf{mod}}}
\newcommand{\gotv}{\ensuremath{\mathsf{gotv}}}

\makeatother


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "book"
%%% End:

